Model checking memoryful linear-time logics over one-counter automata

We study complexity of the model-checking problems for LTL with registers (also known as freeze LTL) and for first-order logic with data equality tests over one-counter automata. We consider several classes of one-counter automata (mainly deterministic vs. nondeterministic) and several logical fragments (restriction on the number of registers or variables and on the use of propositional variables for control locations). The logics have the ability to store a counter value and to test it later against the current counter value. We show that model checking over deterministic one-counter automata is PSPACE-complete with infinite and finite accepting runs. By constrast, we prove that model checking freeze LTL in which the until operator is restricted to the eventually operator over nondeterministic one-counter automata is undecidable even if only one register is used and with no propositional variable. As a corollary of our proof, this also holds for first-order logic with data equality tests restricted to two variables. This makes a difference with the facts that several verification problems for one-counter automata are known to be decidable with relatively low complexity, and that finitary satisfiability for the two logics are decidable. Our results pave the way for model-checking memoryful (linear-time) logics over other classes of operational models, such as reversal-bounded counter machines.

==> auxi-pspace-hard-pure.tex <==

\begin{center}
\begin{figure}[htbp]
\begin{picture}(115,55)(0,0)
%
%\unitlength=1mm
%
\setlength{\unitlength}{0.9mm}
\node(Q0)(5,5){$\aloc_0$}
\node(Q1)(15,5){$\aloc_1$}
\drawedge(Q0,Q1){$\mathtt{ifzero}$}
\node(Q1B)(30,5){$\aloc'_1$}
\drawedge(Q1,Q1B){$\mathtt{inc}$}
\node(Q11)(37,20){$\aloc^1_1$}
\drawedge(Q1B,Q11){$\mathtt{dec}$}
\node(Q2)(45,5){$\aloc_2$}
\drawedge(Q11,Q2){$\mathtt{zero}$}
\node(Q2B)(60,5){$\aloc'_2$}
\drawedge(Q2,Q2B){$\mathtt{inc}$}
\node(Q21)(67,20){$\aloc^1_2$}
\drawedge(Q2B,Q21){$\mathtt{dec}$}
\node(Q22)(67,35){$\aloc^2_2$}
\drawedge(Q21,Q22){$\mathtt{ifzero}$}
\node(Q3)(75,5){$\aloc_3$}
\drawedge[curvedepth=6](Q22,Q3){$\mathtt{ifzero}$}
\node[Nw=0,Nh=0](QT1)(88,5){}
\drawedge[dash={1.5}0](Q3,QT1){$\mathtt{inc}$}
\node[Nw=0,Nh=0](QT2)(92,5){}
\node(Q2NB)(105,5){$\aloc'_{2N}$}
\drawedge[dash={1.5}0](QT2,Q2NB){$\mathtt{inc}$}
\node(Q2N1)(112,20){$\aloc^1_{2N}$}
\drawedge(Q2NB,Q2N1){$\mathtt{dec}$}
\node[Nw=0,Nh=0](Q2N2)(112,35){}
\drawedge[dash={1.5}0](Q2N1,Q2N2){$\mathtt{ifzero}$}
\node[Nw=0,Nh=0](Q2N3)(112,40){}
\node(Q2N2N)(112,53){$\aloc^{2N}_{2N}$}
\drawedge[dash={1.5}0](Q2N3,Q2N2N){$\mathtt{ifzero}$}
\node(QF)(120,5){$\aloc_F$}
\drawedge[curvedepth=6](Q2N2N,QF){$\mathtt{ifzero}$}
\node(QFB)(135,5){$\aloc'_F$}
\drawedge(QF,QFB){$\mathtt{inc}$}
\node(QFBB)(135,25){$\aloc''_F$}
\drawedge(QFB,QFBB){$\mathtt{dec}$}
\drawedge[curvedepth=6](QFBB,QFB){$\mathtt{inc}$}

%
\end{picture}
\caption{Another automaton to simulate $2N$ quantifications}
\label{fig:QBF2}
\end{figure}
\end{center}
%
In the above proof, the alphabet is used in some essential way. Below we show that even the pure
version of the problems (i.e. with no atomic formulae from the alphabet) is \pspace-hard.
Consider the deterministic one-counter automaton $\aautomaton_{\aformula}'$ 
from Figure~\ref{fig:QBF2} in which we have
omitted $\mathtt{ifzero}$ and $\mathtt{dec}$ transitions that lead to a sink location
(these transitions are actually never fired). The only accepting location 
is $\aloc'_F$ and the initial location is $\aloc_0$. 
The  sequence of counter values from the unique infinite accepting run
has the form below:
$$
0 \ 0 \ 1 \ 0 \ 0 \ 1 \ 0 \ 0 \ 0 \ 1 \cdots 0^{2N} 1 \  0^{2N+1} 1 (0 \ 1)^{\omega}
$$

In order to define $\aformulabis'$, we introduce below another 
family of formulae $\aformulabis'_1, \ldots,
\aformulabis'_{2N+1}$ with $\aformulabis' = \aformulabis_1'$ such that 
$\aformulabis'_i$ is obtained from $\aformulabis_i$ by replacing
\begin{itemize}
\itemsep 0 cm
\item $\aloc_F$ by $\downarrow_{2N+1} 
      \big[\mynext \neg \uparrow_{2N+1}  ~\wedge~ \mynext^2  \uparrow_{2N+1} 
        ~\wedge~ \mynext^3 \neg \uparrow_{2N+1}  ~\wedge~ \mynext^4 \uparrow_{2N+1} 
       \big]$,
\item each $\aloc_i$ by
      $
     \downarrow_{2N+1} \big[ \mynext \big( \neg \uparrow_{2N+1}  \bigwedge_{j=1}^{i+1} \mynext^j 
      \uparrow_{2N+1} ~\wedge~ \mynext^{i+2} \neg \uparrow_{2N+1}  \big)]$,
\item  each $\aloc_i'$  by
      $
     \downarrow_{2N+1} \big[ \mynext \big(\neg \uparrow_{2N+1}  \bigwedge_{j=1}^{i} \mynext^j 
      \neg \uparrow_{2N+1} ~\wedge~ \mynext^{i+1} \uparrow_{2N+1}  \big)]$,
\end{itemize}
Similarly, one can show that
$\aformula$ is satisfiable iff
$\aautomaton_{\aformula}' \models^{< \omega} \aformulabis'$ iff
$\aautomaton_{\aformula}' \models^{\omega} \aformulabis'$. 


==> ex-algo-mc.tex <==
The last preliminary property we need before defining the model-checking algorithm
is related to the satisfaction of formulae whose outermost connective is $\until$. 
Indeed, roughly speaking, in order to satisfy $\aformula_1 \until \aformula_2$ at
symbolic context $\pair{i}{\asymbregval}$, we need to find some future 
symbolic context
$\pair{i'}{\asymbregval'}$ satisfying $\aformula_2$ and the symbolic contexts in between
should satisfy $\aformula_1$. The lemma below states that only a polynomial amount 
of possibilities needs to be taken into account.

\begin{lemma} \label{lemma-until}
Let $\pair{i}{\asymbregval}$ be a symbolic
context. There is $K_4$ polynomial in $\length{\locs}$ such that 
for every $\alpha \geq K_4$,
 there is $\beta < K_4$ 
            such that
           $$
           \pair{\set{\move(\pair{i}{\asymbregval},j): 0 \leq j \leq \alpha-1}}{
                 \move(\pair{i}{\asymbregval},\alpha)} =
           $$
           $$
           \pair{\set{\move(\pair{i}{\asymbregval},j): 0 \leq j \leq \beta-1}}{
                 \move(\pair{i}{\asymbregval},\beta)}
           $$
\end{lemma}


\iffossacs
The proof is in Appendix~\ref{section-proofs-section-pspace}.
\else
\begin{proof}
\input{proof-lemma-until}
\qed
\end{proof}
\fi 

As explained earlier, the model-checking algorithm (see Figure~\ref{figure-algorithm}) 
takes as arguments
a deterministic one-counter automaton (encoding the infinite run 
$\arun_{\aautomaton}^{\omega}$), a formula to satisfy and a symbolic context
(we assume implicitly that $N$ registers are involved, otherwise we can add
$N$ as an argument). 


\begin{figure}
$\mc(\aautomaton, \aformulabis, \pair{i}{\asymbregval})$
\begin{itemize}
\itemsep 0 cm
\item $\aformulabis = \uparrow_r $: Return 
      (($0 \in \asymbregval(r)$ and $K_3 > 0$) or ($n_i = \asymbregval(r)$ and $K_3 = 0$));
\item $\aformulabis = \aloc$: Return $\aloc = \aloc_i$;
\item $\aformulabis = \aformulabis_1 \wedge \aformulabis_2$:
      Return ($\mc(\aautomaton, \aformula, \aformulabis_1, \pair{i}{\asymbregval})$
             and $\mc(\aautomaton, \aformulabis_2, \pair{i}{\asymbregval})$);
\item $\aformulabis = \neg \aformulabis_1$:
      Return not $\mc(\aautomaton,  \aformulabis_1, \pair{i}{\asymbregval})$;
\item $\aformulabis = \downarrow_r \aformulabis_1$:
      Return $\mc(\aautomaton,  \aformulabis_1, \pair{i}{\asymbregval'})$
      where $\asymbregval'$ is defined as follows.
      \begin{enumerate}
      \item $\asymbregval'(r') = \asymbregval(r')$ for $r' \neq r$ and
      \item $\asymbregval'(r) = {\rm pos}_{\aautomaton}(i,n_i)$ if $K_3 > 0$.
      \item $\asymbregval'(r) = n_i$ if $K_3 = 0$.
      \end{enumerate}
\item  $\aformulabis = \mynext \aformulabis_1$:
      Return $\mc(\aautomaton,  \aformulabis_1, \move(\pair{i}{\asymbregval},1))$;
\item $\aformulabis = \aformulabis_1 \until \aformulabis_2$: If there is
      $j < K_4$ such that
      \begin{enumerate}
      \item $\mc(\aautomaton,  \aformulabis_2, \move(\pair{i}{\asymbregval},j)) = \top$;
      \item For $0 \leq j' < j$, 
             $\mc(\aautomaton,  \aformulabis_1, \move(\pair{i}{\asymbregval},j')) = \top$;
      \end{enumerate}
      Return $\top$, otherwise Return $\perp$. 
\end{itemize}
\label{figure-algorithm}
\caption{A symbolic model-checking algorithm}
\end{figure}

\begin{lemma} 
Let $\aautomaton$ be a deterministic one-counter automaton and
$\arun_{\aautomaton}^{\omega}$ be its infinite run. 
$\aautomaton \models_{\omega} \aformula$ iff
$\mc(\aautomaton, \aformula, \pair{0}{\asymbregval_0})$ returns true where
$\asymbregval_0$ is the symbolic register valuation representating the zero register valuation. 
\end{lemma}

Observe that $K_1$, $K_2$, $K_3$, $K_4$ and
the $K_1 + K_2$ first configurations of the infinite run can be preprocessed
before applying $\mc$. 


\begin{proof}(sketch) 
The main ingredients of the proof are the following:
\begin{itemize}
\itemsep 0 cm
\item Lemma~\ref{lemma-two-in-one}(I) states that $\equiv$-equivalent contexts
      satisfy the same formulae with at most $N$ registers.
      Consequently, we can work with symbolic contexts that encode concisely
      equivalence classes of contexts.
\item Lemma~\ref{lemma-move} states that moving along $\arun_{\aautomaton}^{\omega}$
      can be done symbolically.
\item The different cases in $\mc$ are quite obvious except for subformulae with
      outermost temporal connective $\until$.
      Lemma~\ref{lemma-until} states that there is no need to look for witness positions
      at distance more than $K_4$ from the current context. 
\end{itemize}
\qed
\end{proof}


==> ex-presburger.tex <==

\subsection{Finitary model-checking over deterministic one-counter automata}

%% 
%% {\it Stephane: I think we can improve what is below. Here are just the ideas.
%% 
%% \begin{lemma} If $\aautomaton \models_{< \omega} \aformula$, then there is a finite accepting
%% run of length polynomial in $\length{\aautomaton} + \length{\aformula}$  satisfying $\aformula$.
%% \end{lemma}
%% 
%% I have not yet the formal but the idea would be to consider witness positions along the
%% finite run (witnessing the (un)satisfaction of temporal formulae) and to shorten 
%% the run accordingly. Some technical details need to be fixed.
%% 
%% Consequently, we would also obtain that for a finite amount registers, the finitary
%% problem is in \ptime: Check the satisfaction of a polynomial amount of finite runs
%% with a polynomial amount of register valuations.
%% 
%% I will think about the proof of the above lemma but here is below a simple decidability
%% proof that we do not believe to be optimal.
%% 
%% }

In this section, we show that 
$\fMC{< \omega}{}$ restricted to deterministic one-counter automata
 can be reduced in polynomial-time to the satisfiability problem for Presburger arithmetic~\cite{Presburger29}
that is known to be complete for double exponential time with  alternating Turing machines 
using a linear amount of alternations, see e.g.~\cite{Berman80}. 
We cannot use the proof for the infinitary case since so far we have no means to bound the length
of the finite accepting runs verifying the formula. Additionnally,  the abstraction performed previously is unsound
in the finite case since two positions after $K_1$ separated by a distance $K_2$ do not have necessarily
the same future. 

Alternatively, the proof below is based on two properties: the unique run of each automaton is definable in Presburger arithmetic
and LTL with registers can be translated in Presburger arithmetic. For instance, the decidability proof below
can be extended to the case when constraints between registers are formulae from Presburger arithmetic instead
of equality tests only (even in the infinitary case).  Moreover, we can enrich the logical language with past-time
operators or with any first-order definable operator and still be able to perform the translation. The details
for these extensions are omitted herein because of lack of space. 
Observe that the infinitary case can be also encoded in such a way in Presburger arithmetic but it is not optimal
in terms of complexity since the problem is \pspace-complete as shown previously.


Let us briefly state the main steps of the decidability proof. 
Let $\arun_{\aautomaton}^{\omega} = \pair{\aloc_0}{n_0} \ \pair{\aloc_1}{n_1} \ \pair{\aloc_2}{n_2} \ldots$ 
be the unique run of the deterministic one-counter
automaton $\aautomaton$ and $\aformula$ be a sentence with $N \geq 1$ registers.
Thanks to Lemma~\ref{lemma-KKK}, the result below is obvious.


\begin{lemma} Given a deterministic one-counter automaton $\aautomaton$, one can effectively
compute a Presburger formula $\apformula(\avariable, \avariablebis, \avariableter)$ (in polynomial-time)
with free variables $\avariable$, $\avariablebis$, $\avariableter$ such that
$$
\set{\triple{a}{b}{c} \in \Nat^3: \triple{a}{b}{c} \models 
\apformula(\avariable, \avariablebis, \avariableter)} =
\set{\triple{i}{n_i}{q_i} \in \Nat^3: i \geq 0}
.
$$
(we identify $\locs$ with a finite set of natural numbers)
\end{lemma}

Since
$\aformula$ has no free register, $\aautomaton \models^{< \omega} \aformula$ iff
there is $i \geq 0$ such that  
$$\pair{\aloc_0}{n_0} \ \pair{\aloc_1}{n_1} \cdots  \pair{\aloc_i}{n_i}, 0 
\models_{\aregval_0} \aformula,$$
$\pair{\aloc_0}{n_0} \ \pair{\aloc_1}{n_1} \cdots  \pair{\aloc_i}{n_i}$ is an accepting run
and $\aregval_0$ assigns $0$ to every register in $\set{1,\ldots,N}$. 

The translation map $\atranslation$ admits the following arguments:
the subformula $\aformulabis$ to be translated,
$\avariable$ interpreted as the current position in the run,
$\vect{\avariablebis} = \avariablebis_1, \ldots, \avariable_N$ interpreted as the register values
and $\avariable_{end}$ interpreted as the last position of the run.
Here is its inductive definition. 
\begin{itemize}
\itemsep 0 cm
\item $\atranslation(\aloc, \avariable, \vect{\avariablebis}, \avariable_{end})
       = \exists \ \avariablebis', \avariableter' \ 
         \apformula(\avariable, \avariablebis', \avariableter') \wedge \avariableter' = \aloc$,
\item  $\atranslation(\uparrow_r , 
         \avariable, \vect{\avariablebis}, \avariable_{end})
       = \exists \ \avariablebis', \avariableter' \ 
         \apformula(\avariable, \avariablebis', \avariableter') \wedge 
       \avariablebis' = \avariablebis_r$,
\item $\atranslation$ is homomorphic for Boolean operators,
\item  $\atranslation(\downarrow_r \aformulabis, 
         \avariable, \vect{\avariablebis}, \avariable_{end})
       = \exists \ \avariablebis', \avariableter' \ 
         \apformula(\avariable, \avariablebis', \avariableter') \wedge 
          \atranslation(\aformulabis, 
         \avariable, \avariablebis_1, \ldots,\avariablebis_{r-1}, \avariablebis',
          \avariablebis_{r+1}, \ldots, \avariablebis_N, \avariable_{end})$,
\item $\atranslation(\mynext \aformulabis, 
         \avariable, \vect{\avariablebis}, \avariable_{end})
       = \exists \ \avariable' \
         \avariable' = \avariable + 1 \wedge
          \avariable' \leq \avariable_{end} \wedge 
          \atranslation(\aformulabis, 
         \avariable', \vect{\avariablebis}, \avariable_{end})$
\item $\atranslation(\aformulabis_1 \until \aformulabis_2, 
         \avariable, \vect{\avariablebis}, \avariable_{end})
       = \exists \ \avariable' \
         \avariable \leq \avariable' \leq \avariable_{end} \wedge 
          \atranslation(\aformulabis_2, 
                        \avariable', \vect{\avariablebis}, \avariable_{end}) \wedge
           (\forall \avariable'' \ 
            (\avariable \leq \avariable'' < \avariable') \Rightarrow 
            \atranslation(\aformulabis_1, 
                        \avariable'', \vect{\avariablebis}, \avariable_{end}))$.
\end{itemize}


\begin{lemma}
$\aautomaton \models^{< \omega} \aformula$ iff
the formula below
$$ \aformula' = 
\exists \ \avariable_{end} \
\exists \ \avariable, \avariablebis_1, \ldots, \avariablebis_N \
(
\atranslation(\aformula, \avariable, \avariablebis_1, \ldots, \avariablebis_N, \avariable_{end})
\ \wedge \
\overbrace{\avariable = \avariablebis_1 = \cdots =\avariablebis_N = 0}^{\rm initial \ values}
\ \wedge
$$
$$
\underbrace{
(\exists \avariablebis', \avariableter' \ 
        \apformula(\avariable_{end}, \avariablebis', \avariableter') \wedge 
        (\bigvee_{\aloc \in F} \avariableter' = \aloc))}_{\rm run \ ends \ in \ F}
)
$$
holds true in Presburger arithmetic.
\end{lemma}

Observe that $\aformula'$ is in polynomial size in $\length{\locs} + \length{\aformula}$.
The tedious proof simply takes advantage of the fact that $\atranslation$ encodes the first-order semantics of
$\fLTL{\downarrow,\aalphabet}{}$ and any finite accepting run is definable in Presburger arithmetic. 


\begin{theorem} 
$\fMC{< \omega}{}$ restricted to deterministic one-counter automata is decidable
and it can be solved in double exponential time with an alternating Turing machine 
using a linear amount of alternations.
\end{theorem}

The above translation is reminiscent to translations into Presburger arithmetic performed
in~\cite{Bruyere&DallOlio&Raskin03,Demrietal06} but does not allow us to characterize complexity of this
finitary  variant. Even though \pspace-hardness can be established by slightly
adapting arguments from Sect.~\ref{section-pspace-lower-bound}, the existence
of an \pspace \ upper bound is open. 
We conjecture that if $\aautomaton \models^{< \omega} \aformula$, then there is a finite accepting
 run of length at most exponential in $\length{\aautomaton} + \length{\aformula}$  satisfying 
$\aformula$.
 

==> ex-proof-pspace-hardness.tex <==
\begin{proof} Consider a \QBF \ instance $\aformula$:
%
$
\aformula = 
\forall \avarprop_1 \
\exists \avarprop_2 \ \cdots \
\forall \avarprop_{2N-1} \ \exists \ \avarprop_{2N} \ \Psi(\avarprop_1,...,\avarprop_{2N})
$
%
where  $\avarprop_1$,...,$\avarprop_{2N}$ are propositional variables and 
$\Psi(\avarprop_1, \ldots,\avarprop_{2N})$ is a quantifier-free propositional 
formula built over $\avarprop_1, \ldots, \avarprop_{2N}$.
Fig.~\ref{fig:QBF} contains the definition of the deterministic one-counter automaton
$\aautomaton_{\aformula}$ with $\aloc_F$ the unique accepting location and $\aloc_0$ is the
initial location. 
The sequence of the $2N+2$th first counter values is precisely
$0(01)^{2N}0$. 
This will allow us to simulate quantifications in $\aformula$  by using
alternatively
the temporal operators $\sometimes$ and $\always$. 
Below, value ``$1$'' stands for the truth constant ``$\top$''.





%
\begin{center}
\begin{figure}[htbp]
\begin{picture}(115,15)(-5,0)
\setlength{\unitlength}{0.9mm}
%
%\unitlength=1mm
%
\node(Q0)(-3,5){$\aloc_0$}
\node(Q1)(20,5){$\aloc_1$}
\drawedge(Q0,Q1){$\mathtt{ifzero}$}
\node(Q1B)(35,5){$\aloc'_1$}
\drawedge(Q1,Q1B){$\mathtt{inc}$}
\node(Q2)(50,5){$\aloc_2$}
\drawedge(Q1B,Q2){$\mathtt{dec}$}
\node(Q2B)(65,5){$\aloc'_2$}
\drawedge(Q2,Q2B){$\mathtt{inc}$}
\node(Q3)(80,5){$\aloc_3$}
\drawedge(Q2B,Q3){$\mathtt{dec}$}
\node[Nw=0,Nh=0](QT1)(93,5){}
\drawedge[dash={1.5}0](Q3,QT1){$\mathtt{inc}$}
\node[Nw=0,Nh=0](QT2)(97,5){}
\node(Q2NB)(110,5){$\aloc'_{2N}$}
\drawedge[dash={1.5}0](QT2,Q2NB){$\mathtt{inc}$}
\node(QF)(125,5){$\aloc_F$}
\drawedge(Q2NB,QF){$\mathtt{dec}$}
\drawloop(QF){$\mathtt{ifzero}$}
%
\end{picture}
\caption{An automaton to simulate $2N$ quantifications}
\label{fig:QBF}
%
\end{figure}
\end{center}
%

Let $\aformulabis$ be the formula in $\fLTL{\downarrow,\aalphabet_{2N}}{2N}$ with
$\aalphabet_{2N} = \set{\aloc_0,\aloc_1,\aloc_1', \ldots,\aloc_{2N},\aloc'_{2N},\aloc_F}$.  
In order to define $\aformulabis$, we introduce below a family of formulae $\aformulabis_1, \ldots,
\aformulabis_{2N+1}$ with $\aformulabis = \aformulabis_1$. 
%
\begin{itemize}
\itemsep 0 cm
\item $\aformulabis_{2N+1} =\sometimes \big(\aloc_F \wedge 
      \Psi[\avarprop_i \leftarrow \neg \uparrow_i] \big)$,
\item for all $i \in \set{1,...,N}$, 
      $\aformulabis_{2i} = \sometimes \big( (\aloc_{2i} \vee \aloc'_{2i}) 
                        \wedge \downarrow_{2i} \mynext \aformulabis_{2i+1}\big)$, 
\item for all $i \in \set{0,...,N-1}$, $\aformulabis_{2i+1}= \always 
       \big( (\aloc_{2i+1} \vee \aloc'_{2i+1}) \Rightarrow \downarrow_{2i+1} 
       \mynext \aformulabis_{2i+2}\big)$. 
\end{itemize}
%
One can show that the equivalences below: 
\begin{center}
$\aformula$ is satisfiable iff $\aautomaton_{\aformula} \models_{< \omega} \aformulabis$ iff
$\aautomaton_{\aformula} \models_{\omega} \aformulabis$. 
\end{center}
To do so, we proceed as follows. For $i \in \set{0,2,4,6,\ldots,2N}$, let $\aformula_i$ be
$$
\aformula_i = 
\forall \avarprop_{i+1} \
\exists \avarprop_{i+2} \ \cdots \
\forall \avarprop_{2N-1} \ \exists \ \avarprop_{2N} \ \Psi(\avarprop_1,...,\avarprop_{2N}).
$$
So $\aformula_0$ is precisely $\aformula$. 
Similarly, for 
 $i \in \set{1,3,5,\ldots,2N-1}$, let $\aformula_i$ be
$$
\aformula_i = 
\exists \avarprop_{i+1} \
\forall \avarprop_{i+2} \ \cdots \
\forall \avarprop_{2N-1} \ \exists \ \avarprop_{2N} \ \Psi(\avarprop_1,...,\avarprop_{2N}).
$$
Observe that the free propositional variables in $\aformula_i$ are precisely $\avarprop_1,
\ldots, \avarprop_{i}$ and $\aformula_i$ is obtained from $\aformula$ by removing the $i$th first 
quantifications. 
Given a propositional valuation $\aregval: \set{\avarprop_1, \ldots,
\avarprop_i} \rightarrow \set{\top,\perp}$ for some $i \in \set{1, \ldots,2N}$,
we write $\overline{\aregval}$ to denote a register valuation such that its restriction
to $\set{1,\ldots,i}$ satisfies: $\aregval(\avarprop_j) = \top$ iff $\overline{\aregval}(j) = 
1$ for $j \in \set{1,\ldots,i}$. One can show by induction that 
$\aregval \models \aformula_{i-1}$ (in \QBF) iff
$\arun_{\aautomaton}^{\omega}, 2i-2 \models_{\overline{\aregval}}  \aformulabis_{i}$.
Consequently, if $\aregval \models \aformula$ for some propositional valuation, then
$\arun_{\aautomaton}^{\omega}, 0 \models_{\overline{\aregval}}  \aformulabis$.
Similarly, if $\arun_{\aautomaton}^{\omega}, 0 \models_{\aregval}  \aformulabis$, then
there is a propositional valuation $\aregval'$ such that
$\overline{\aregval'} = \aregval$ and $\aregval' \models \aformula$.
\qed
%% \\$\Box$
%% Ste 150807
%% We will build the one-counter machine $M_{\Psi}$ represented in figure \ref{fig:QBF}. 
%% We first note that this one-counter machine is deterministic. We build then a \freezeLTLdef 
%% formula $\Phi$ inductively as follows~:
%% %
%% \begin{itemize}
%% \item $\Phi_{2N+1}=\textsf{F} \big(q_F \wedge \Psi[X_i \leftarrow \uparrow_i] \big)$
%% \item for all $i \in \{1,...,N\}$, $\Phi_{2i}=\textsf{F} \big( (q_{2i} \vee q'_{2i}) \wedge 
%% \downarrow_{2i} \Phi_{2i+1}\big)$ 
%% \item for all $i \in \{0,...,N-1\}$, $\Phi_{2i+1}=\textsf{G} \big( (q_{2i+1} \vee q'_{2i+1}) 
%% \Rightarrow \downarrow_{2i+1} \Phi_{2i+2}\big)$ 
%% \item $\Phi=\Phi_1$
%% \end{itemize}
%% %
%% 
%% We will show that the formula of \textsf{QBF} $\forall X_1.\exists X_2.~...~.\forall X_{2N-1}.\exists 
%% X_{2N}. \Psi(X_1,...,X_{2N})$ is satisfiable if and only if $M_{\Psi} \models_I \Phi$.
%% \\$\Box$
\end{proof}


==> ex-purification.tex <==

In this section, we show how to get rid of propositional variables
by reducing 
the model checking problem over one-counter automata to its pure version.
Let $\aautomaton=\triple{\locs,\aloc_I}{\delta}{F}$ be a one-counter automaton
with $\locs=\set{\aloc_1,...,\aloc_n}$ and
$\aformula$ be a sentence in $\fLTL{\downarrow,Q}{}$.
We shall 
build a one-counter automaton $\aautomaton_{P}=\triple{\locs',\aloc_I}{\delta}{F'}$ and a 
sentence $\phi_P \in \fLTL{\downarrow,\emptyset}{}$ such that 
$\aautomaton \models^\alpha \aformula$ iff $\aautomaton_P \models^{\alpha} \aformula_P$. 
The main idea is to identify locations with patterns about the changes of the unique counter.
To do so, we complete $\aautomaton$ in order to characterize each of its location 
with a unique formula of $\fLTL{\downarrow,\emptyset}{}$.


Intuitively, the sets $Q'$ and $\delta'$ are  built following Fig.~\ref{fig:purif1}.
%%  (or figure \ref{fig:purif2})
We replace each location $\aloc_i \in \locs$ 
by $i$ successive increasing picks as shown in Fig.~\ref{fig:purif1}.
Moreover, for each transition $\aloc_i \step{a} \aloc_j \in \delta$, 
we add a transition $\aloc^F_i \step{a} \aloc_j$ to $\delta'$.  Finally, 
the new set of accepting locations is $F'= \set{\aloc^F_i \mid \aloc_i \in F}$. 
Note that determinisn is preserved by this transformation.\\

%% Ste 031007
%% %
%% To build the formula $\aformula_P$, 
%% we first define a family of formulae $\set{\phi_i}_{1 \leq i \leq n}$ such that~:
%% $$
%% \aformula_i=\downarrow_1 \big ( \mynext^2 \uparrow_1 \wedge 
%% \bigwedge_{1 \leq j \leq i} \mynext^{f(j)} \uparrow_1)
%% $$
%% where $f(1)=6$ and for all $j>1$, $f(j)=f(j-1)+2.j+2$. 
%% We write {\rm LOC} to denote
%% the formula $\bigvee_{1 \leq i \leq n} \aformula_i$.\\
%% %%  and $r$ can be any register used in the formula $\phi$.\\
To build the formula $\aformula_P$, 
we first define a family of formulae $\set{\aformula_i}_{1 \leq i \leq n}$ 
such that~:
 $$
 \aformula_i= \downarrow_1  \bigwedge_{1 \leq j \leq i} \mynext^{(j+1)j}
              \uparrow_1
$$
We write {\rm LOC} to denote
the formula $\bigvee_{1 \leq i \leq n} \aformula_i$.\\
%% %%  and $r$ can be any register used in the formula $\phi$.\\
% %

The formula $\aformula_P$ is defined as 
$\atranslation(\aformula)$ with the map 
$\atranslation$ that is homomorphic for 
Boolean operators and $\downarrow_r$, and its restriction to $\uparrow_r$ is identity. 
The rest of the inductive definition of the map $\atranslation$ is the following~:
\begin{itemize} 
\itemsep 0 cm
\item $\atranslation(\aloc_i)= \aformula_i \wedge \bigwedge_{j \in \set{1,\ldots,n} \setminus \{i\}} \neg \aformula_j$
\item  $\atranslation(\aformula \until \aformula')=
       \big ({\rm LOC} \Rightarrow \atranslation(\aformula) \big) 
\until \big ({\rm LOC} \wedge \atranslation(\aformula') \big )$
\item $\atranslation(\mynext \aformula) =\mynext \big ( (\neg {\rm LOC}) 
      \until ({\rm LOC} \wedge \atranslation(\aformula))\big)$.
\end{itemize}
%
We remark that $\aformula$ and $\aformula_P$ have the same amount of registers unless
$\aformula$ has no register. 
% we do not need any additional register to build the formula $\aformula_P$.\\
This leads to the following lemma.
%
\begin{lemma}[Purification]
\label{lemma-purification}
Given a one-counter automaton $\aautomaton$
              and  a sentence $\aformula$ in 
              $\fLTL{\downarrow,\locs}{}$, one can compute in logarithmic space in
$\length{\aautomaton} + \length{\aformula}$ a one-counter automaton 
$\aautomaton_P$ and $\aformula_P$ in $\fLTL{\downarrow,\emptyset}{}$  such that  $\aautomaton \models^{< \omega} \aformula$
                 [resp. $\aautomaton \models^{\omega} \aformula$ ] iff 
$\aautomaton_P \models^{< \omega} \aformula_P$
                 [resp. $\aautomaton_P \models^{\omega} \aformula_P$].
Moreover, $\aautomaton$ is deterministic 
% [resp. weakly deterministic] 
iff $\aautomaton'$  is deterministic.
% [resp. weakly deterministic]. 
\end{lemma}
%
\begin{center}
\begin{figure}[htbp]
\begin{picture}(130,50)(5,0)
%
%\unitlength=1mm
%
\setlength{\unitlength}{0.9mm}
\node(Q)(5,5){$\aloc_i$}
\node(Q0)(15,18){$\aloc^0_i$}
\drawedge(Q,Q0){$\mathtt{inc}$}
\node(Q11)(25,5){$\aloc^{1,1}_1$}
\drawedge[ELside=r](Q0,Q11){$\mathtt{dec}$}
\node(Q12)(35,18){$\aloc^{1,2}_i$}
\drawedge(Q11,Q12){$\mathtt{inc}$}
\node(Q13)(40,31){$\aloc^{1,3}_i$}
\drawedge(Q12,Q13){$\mathtt{inc}$}
\node(Q14)(45,18){$\aloc^{1,4}_i$}
\drawedge(Q13,Q14){$\mathtt{dec}$}
\node(Q21)(55,5){$\aloc^{2,1}_i$}
\drawedge[ELside=r](Q14,Q21){$\mathtt{dec}$}
\node(Q22)(65,18){$\aloc^{2,2}_i$}
\drawedge(Q21,Q22){$\mathtt{inc}$}
\node(Q23)(70,31){$\aloc^{2,3}_i$}
\drawedge(Q22,Q23){$\mathtt{inc}$}
\node(Q24)(75,44){$\aloc^{2,4}_i$}
\drawedge(Q23,Q24){$\mathtt{inc}$}
\node(Q25)(80,31){$\aloc^{2,5}_i$}
\drawedge(Q24,Q25){$\mathtt{dec}$}
\node(Q26)(85,18){$\aloc^{2,6}_i$}
\drawedge(Q25,Q26){$\mathtt{dec}$}
\node(Q31)(95,5){$\aloc^{3,1}_i$}
\drawedge[ELside=r](Q26,Q31){$\mathtt{dec}$}
\node[Nw=0,Nh=0](QT1)(104,16){}
\drawedge[dash={1.5}0](Q31,QT1){$\mathtt{inc}$}
\node[Nw=0,Nh=0](QT2)(116,29){}
\node[Nadjust=w](QF1)(120,18){$\aloc^{i,2.i+2}_i$}
\drawedge[dash={1.5}0](QT2,QF1){$\mathtt{dec}$}
\node(QF)(125,5){$\aloc^{F}_i$}
\drawedge[ELside=r](QF1,QF){$\mathtt{dec}$}
%\node(Qj)(140,5){$\aloc_j$}
%\drawedge(QF,Qj){$a$}
%
\end{picture}
\caption{Encoding $\aloc_i$ by a pattern made of $i$ increasing picks}
\label{fig:purif1}
\end{figure}
\end{center}

%%
%%
%%\input{figure-2}
%%

==> figure-2.tex <==
%
\begin{center}
\begin{figure}[htbp]
\begin{picture}(120,50)(5,0)
%
%\unitlength=1mm
%
\setlength{\unitlength}{0.9mm}
\node(Q)(5,5){$\aloc_i$}
\node(Q0)(15,18){$\aloc^0_i$}
\drawedge(Q,Q0){$\mathtt{inc}$}
\node(Q11)(25,5){$\aloc^{1,1}_1$}
\drawedge[ELside=r](Q0,Q11){$\mathtt{dec}$}
\node[Nw=0,Nh=0](Q12)(33,16){}
\drawedge[dash={1.5}0](Q11,Q12){$\mathtt{inc}$}
\node[Nw=0,Nh=0](Q14)(37,17){}
\node(Qj1)(45,5){$\aloc^{k,1}_i$}
\drawedge[ELside=r,dash={1.5}0](Q14,Qj1){$\mathtt{dec}$}
\node(Qj2)(55,18){$\aloc^{k,2}_i$}
\drawedge(Qj1,Qj2){$\mathtt{inc}$}
\node[Nw=0,Nh=0](Qj3)(60,29){}
\drawedge[dash={1.5}0](Qj2,Qj3){$\mathtt{inc}$}
\node[Nw=0,Nh=0](Qj4)(62,33){}
\node[Nadjust=w](Qj5)(68,44){$\aloc^{k,k+2}_i$}
\drawedge[ELpos=40,dash={1.5}0](Qj4,Qj5){$\mathtt{inc}$}

\node[Nw=0,Nh=0](Qj6)(72,33){}
\drawedge[ELpos=60,dash={1.5}0](Qj5,Qj6){$\mathtt{dec}$}
\node[Nw=0,Nh=0](Qj7)(75,29){}
\node[Nadjust=w](Qj8)(80,18){$\aloc^{k,2.k+2}_i$}
\drawedge[ELpos=40,dash={1.5}0](Qj7,Qj8){$\mathtt{dec}$}
\node[Nadjust=w](Qj9)(90,5){$\aloc^{k+1,1}_i$}
\drawedge[ELside=r,ELpose=60](Qj8,Qj9){$\mathtt{dec}$}
\node[Nw=0,Nh=0](Qj10)(98,16){}
\drawedge[ELpos=50,dash={1.5}0](Qj9,Qj10){$\mathtt{inc}$}
\node[Nw=0,Nh=0](QT2)(106,29){}
\node[Nadjust=w](QF1)(110,18){$\aloc^{i,2.i+2}_i$}
\drawedge[dash={1.5}0](QT2,QF1){$\mathtt{dec}$}
\node(QF)(115,5){$\aloc^{F}_i$}
\drawedge[ELside=r](QF1,QF){$\mathtt{dec}$}
%\node(Qj)(130,5){$\aloc_j$}
%\drawedge(QF,Qj){$a$}
%
\end{picture}
\caption{Transformation of $\aloc_i$ for the purification}
\label{fig:purif2}
\end{figure}
\end{center}%





==> infinitary-pure.tex <==

% \subsection{Infinitary model-checking problems}
%

Before showing that $\fMC{\omega}{1}$ is $\Sigma^1_1$-complete, 
we provide a simple reduction from $\omega$-SAT-LTL$^{\downarrow}$ restricted to formulae with one register, see 
Theorem~\ref{th:undecid-ltl}.
Consider the one-counter automaton $\aautomaton_{sat}$ defined in 
 Figure~\ref{fig:sat-undec}. The initial location is $\aloc_I$ and the unique
accepting location is $\aloc_{f}$. 
%
\begin{figure}[htpb]
\begin{center}
\begin{picture}(50,13)(0,0)
%
\setlength{\unitlength}{0.7mm}
\node(1)(10,10){$\aloc_I$}
\node(2)(40,10){$\aloc_f$}

%
\drawedge[curvedepth=8](1,2){$\mathtt{inc}$}
\drawedge[curvedepth=8](2,1){$\mathtt{ifzero}$}
%%
%% Arn 060907
%% \node(3)(25,5){$\aloc_f$}
%%\drawedge[curvedepth=8](3,1){$\mathtt{ifzero}$}
%%
%
\drawloop[loopangle=180](1){$\mathtt{inc}$}
\drawloop[loopangle=0](2){$\mathtt{dec}$}
%
\end{picture}
\end{center}
\caption{An automaton to encode $\omega$-SAT-LTL$^{\downarrow}$ restricted to one register}
\label{fig:sat-undec}
\end{figure}
%

Given a formula $\aformula$ in $\fLTL{\downarrow,\aalphabet}{1}$,
we build the  formula $\atranslation(\aformula)$ in $\fLTL{\downarrow,\aalphabet}{1}$  
as follows where $Pos=\downarrow_1 \mynext^2 \uparrow_1 $~:
%
\begin{itemize}
\itemsep 0 cm
\item $\atranslation$ is 
      homomorphic for Boolean operators and its restriction to atomic formulae is identity,
%%
%% Ste 150807
%% \item $T(a)=a$
%% \item $T(\uparrow_r \sim)=\uparrow_r \sim$
%% \item $T(\neg \phi)=\neg T(\phi)$
%5 \item $T(\phi \wedge \phi')=T(\phi) \wedge T(\phi')$
%% 
\item $\atranslation(\aformula_1 \until \aformula_2) = \big(Pos \Rightarrow 
      \atranslation(\aformula_1)\big) \
        \until \ \big(Pos \wedge \atranslation(\aformula_2)\big)$,
\item $\atranslation(\mynext \aformulabis )= \mynext \big((\neg Pos) \ \until \ 
       (Pos \wedge \atranslation(\aformulabis))\big)$,
\item $\atranslation(\downarrow_1 \aformulabis) = \downarrow_1 \atranslation(\aformulabis)$.
\end{itemize} 
%% Ste 160807
%% %
%% We can then show that the formula $\Phi$ is satisfiable if and only if 
%% $M \not\models_I \neg T(\Phi)$. This allows us to deduce the following lemma~:
%% %
%% 
\begin{lemma}
$\aformula$ has an infinite model iff $\aautomaton_{sat} \models_{\omega} \atranslation(\aformula)$ 
where $\aautomaton_{sat}$
is the one-counter automaton defined in Figure~\ref{fig:sat-undec}.
\end{lemma} 

\begin{proof} Given an infinite 
accepting run $\arun = \pair{\aloc_0}{n_0} \pair{\aloc_1}{n_1} \cdots$ of $\aautomaton_{sat}$,
we write $\adataword^{\arun}$ to denote the infinite data word defined as follows.
Let $i_0 < i_1 < i_2 < \ldots$ be the unique 
infinite strictly increasing sequence of positions such that
$\aloc_{i_j} = \aloc_1$ and $\aloc_{i_{j}+1} = \aloc'$. 
Let $\adataword^{\arun}$ be the data word in $\locs^{\omega}(\sim)$
such that $\tt{str}(\adataword^{\arun}) = \aloc_0 \aloc_1 \aloc_2 \cdots$ 
and $k \sim^{\adataword^{\arun}} k'$ iff $n_{i_k} = n_{i_{k'}}$. 
One can show by structural induction that $\adataword^{\arun}, 0 \models \aformula$
iff $\arun, 0 \models \atranslation(\aformula)$. 
Similarly, given an infinite data word $\adataword$ such that $\adataword, 0 \models \aformula$,
it is possible to build an accepting run $\arun$ such that 
$\adataword^{\arun} = \adataword$ and therefore 
 $\adataword, 0 \models \aformula$
iff $\arun, 0 \models \atranslation(\aformula)$. 
\qed
\end{proof} 

%
Using Theorem~\ref{th:undecid-ltl}, we conclude. 
%
\begin{theorem} $\fpureMC{\omega}{1}$ restricted to the input
one-counter automaton $\aautomaton_{sat}$ 
is $\Pi_1^0$-hard. 
\end{theorem}
%

It is worth observing that in the infinitary case, undecidability holds true even without
alphabet (see \cite{Demri&Lazic&Nowak06} for eliminating alphabet and extra flexible variables).


%% Ste 290907
%% 
%%  Undecidability can be also proved for a stricter class of one-counter automata.
%%  A one-counter automaton $\aautomaton$ is \emph{weakly deterministic} whenever 
%%  for every location $\aloc$, if $\triple{\aloc}{l}{\aloc'}, \triple{\aloc}{l'}{\aloc''}
%%  \in \delta$, we have $l = l'$ implies $\aloc' = \aloc''$. 
%%  Observe that the transition systems induced by weakly deterministic one-counter automata
%%  are not necessarily deterministic.
%% 
%% By Proposition~\ref{prop:wd}, we obtain the following refinement. 
%% %% And by the proposition \ref{prop:wd}, we obtain~:
%% %
%% \begin{theorem}
%% $\fpureMC{\omega}{1}$ restricted to  
%5 weakly deterministic one-counter automata 
%% is $\_1^1$-hard. 
%% \end{theorem}
%





==> mc.tex <==
%
%
In this section, we define the problem of model-checking one-counter machine with \freezeLTLdef formulae.
%
\subsection{Data-words recognized by a one-counter machine}
%
Let $M=\langle  Q, \delta, q_0, F \rangle$ be a one-counter machine. We define the runs of $M$ as the set $\mathcal{R}(M) \subseteq (Q \times \entiers)^{\leq \omega}$ such that $r \in \mathcal{R}(M)$ if and only if~:
\begin{itemize}
\item $r(1)=(q_0,0)$, 
\item and $\forall i \in \{1,...,|r|-1\}$, $r(i) \rightarrow_M r(i+1)$.
\end{itemize}
where $r(i)$ for $i \in \{1,...,|r|-1\}$ represents the $i$-th configuration in the run and $|r|$ represents the (possibly infinite) size of the run.
We define the projection functions $loc : Q \times \entiers \rightarrow Q$ and $val : Q \times \entiers \rightarrow \entiers$ over the configurations of $M$.  We denote by $\mathcal{R}_F(M)$ the set of finite accepted runs of $M$. A run $r$ is a finite accepted run of $M$ if and only if there exists $n \in \entiers$ such that $n=|r|$ and $loc(r(n)) \in F$. And $\mathcal{R}_I(M)$ will denote the set of infinite accepted runs of $M$, this means the runs $r$ such that the set $\{i \in \entiers \mid loc(r(i)) \in F\}$ is infinite. 

%
The functions $loc$ and $val$ can be extended in an obvious way to runs of $M$ in order to obtain words of control states and words of integers. The data words recognized by $M$ is the set $\mathcal{W}(M)$ defined by $(\sigma,\sim^\sigma) \in \mathcal{W}(M)$ if and only if there exists a run $r \in \mathcal{R}(M)$ such that~:
\begin{itemize}
\item $\sigma=loc(r)$,
\item and for all $0 \leq i,j \leq |\sigma|$, $i \sim^\sigma j$ if and only if 
      $val(r(i))=val(r(j))$.
\end{itemize}
%
$\mathcal{W}_F(M)$ (respectively $\mathcal{W}_I(M)$) will then represent the set of finite data words obtained from the finite (respectively infinte) accepted runs.

%
We will now define the model-checking problem over one-counter machine with \freezeLTLdef. Let $M=\langle  Q, \delta, q_0, F \rangle$ be a one-counter machine. We take $\Sigma=Q$ as alphabet for the atomic propositions of the formulae. Let $\phi$ be a sentence of \freezeLTLdef. We say that $M$ verifies $\phi$ over finite runs (denoted by $M \models_F \phi$) if and only if or all $(\sigma,\sim^\sigma) \in \mathcal{W}_F(M)$, we have $\sigma,0 \models_v \phi$. And we say that $M$ verifies $\phi$  over infinite run (denoted by $M \models_I \phi$) if and only if for all $(\sigma,\sim^\sigma) \in \mathcal{W}_I(M)$, we have $\sigma,0 \models_v \phi$. 
%

\subsection{Reduction to weakly deterministic one-counter machine}
%
We consider a one-counter machine $M=\langle  Q, \delta, q_0, F \rangle$. And from it we will build a weakly deterministic $M'=\langle  Q', \delta', q_0, F \rangle$ with $Q \subseteq Q'$. The figure \ref{fig:weak-det} shows example on the way to weakly determinized a one-counter machine. The examples given in this figure can easily be generalized to all the transitions of $M$. Suppose then we have a formula $\phi$ of \freezeLTLdef over $M$, we build a formula $T(\phi)$ over $M'$ inductively as follows~:
%
\begin{itemize}
\item $T(a)=a$
\item $T(\uparrow_r \sim)=\uparrow_r \sim$
\item $T(\neg \phi)=\neg T(\phi)$
\item $T(\phi \wedge \phi')=T(\phi) \wedge T(\phi')$
\item $T(\phi \textsf{U} \phi')=\big((\bigvee_{q \in Q} q) \Rightarrow T(\phi)\big) \textsf{U}\big(\bigvee_{q \in Q} q \wedge T(\phi')\big)$
\item $T(\textsf{X} \phi)=\textsf{X}\big((\neg \bigvee_{q \in Q} q) \textsf{U} (\bigvee_{q \in Q} q \wedge T(\phi))\big)$
\item $T(\downarrow_r \phi)=\downarrow_r \phi$
\end{itemize}
%
%
\begin{figure}[htbp]
\begin{picture}(145,90)(0,0)
%
%\unitlength=1mm
%
\node(Q)(5,20){$q$}
\node(Q1)(25,5){$q_1$}
\node(Q2)(25,20){$q_2$}
\node(Q3)(25,35){$q_3$}
%
\drawedge(Q,Q1){$inc$}
\drawedge(Q,Q2){$inc$}
\drawedge(Q,Q3){$inc$}
%
%\node(L1)(35,20){}
%\node(L2)(55,20){}
%\drawedge(L1,L2){}
%\drawedge[NHab=0](L1,L2){}

\drawline[linewidth=0.9,AHLength=4,AHlength=0,AHnb=1](35,20)(60,20)

%
\node(WQ)(65,5){$q$}
\node(A)(80,5){$q_1^1$}
\drawedge(WQ,A){$inc$}
\node(B)(95,5){$q_1^2$}
\drawedge(A,B){$dec$}
\node(C)(110,5){$q_1$}
\drawedge(B,C){$inc$}
%
\node(D)(80,20){$q_2^1$}
\drawedge(A,D){$inc$}
\node(E)(95,20){$q_2$}
\drawedge(D,E){$dec$}
%
\node(F)(80,35){$q_3^1$}
\drawedge(D,F){$inc$}
\node(G)(95,35){$q_3^2$}
\drawedge(F,G){$dec$}
\node(H)(110,35){$q_3$}
\drawedge(G,H){$dec$}
%
\node(DQ)(5,70){$q$}
\node(DQ1)(25,55){$q_1$}
\node(DQ2)(25,70){$q_2$}
\node(DQ3)(25,85){$q_3$}
%
\drawline[linewidth=0.9,AHLength=4,AHlength=0,AHnb=1](35,70)(60,70)
%
\drawedge(DQ,DQ1){$dec$}
\drawedge(DQ,DQ2){$dec$}
\drawedge(DQ,DQ3){$dec$}
%
\node(DWQ)(65,55){$q$}
\node(DA)(80,55){$q^1_1$}
\drawedge(DWQ,DA){$dec$}
\node(DB2)(95,55){$q^2_1$}
\drawedge(DA,DB2){$inc$}
\node(DB3)(110,55){$q_1$}
\drawedge(DB2,DB3){$dec$}
%
\node(DD)(95,70){$q_2^2$}
\drawedge(DB2,DD){$inc$}
\node(DE)(110,70){$q_2^3$}
\drawedge(DD,DE){$dec$}
\node(DB)(125,70){$q_2$}
\drawedge(DE,DB){$dec$}
%
\node(DF)(95,85){$q_3^2$}
\drawedge(DD,DF){$inc$}
\node(DG)(110,85){$q_3^3$}
\drawedge(DF,DG){$dec$}
\node(DH)(125,85){$q_3^4$}
\drawedge(DG,DH){$dec$}
\node(DI)(140,85){$q_3$}
\drawedge(DH,DI){$dec$}
%
\node(ZQ)(5,120){$q$}
\node(ZQ1)(25,105){$q_1$}
\node(ZQ2)(25,120){$q_2$}
\node(ZQ3)(25,135){$q_3$}
%
\drawline[linewidth=0.9,AHLength=4,AHlength=0,AHnb=1](35,120)(60,120)
%
\drawedge(ZQ,ZQ1){$zero$}
\drawedge(ZQ,ZQ2){$zero$}
\drawedge(ZQ,ZQ3){$zero$}
%
\node(ZWQ)(65,105){$q$}
\node(ZA)(80,105){$q^1_1$}
\drawedge(ZWQ,ZA){$zero$}
\node(ZB2)(95,105){$q_1$}
\drawedge(ZA,ZB2){$zero$}

%
\node(ZD)(80,120){$q_2^1$}
\drawedge(ZA,ZD){$inc$}
\node(ZE)(95,120){$q_2^2$}
\drawedge(ZD,ZE){$dec$}
\node(ZB)(110,120){$q_2$}
\drawedge(ZE,ZB){$zero$}
%
\node(ZF)(80,135){$q_3^1$}
\drawedge(ZD,ZF){$inc$}
\node(ZG)(95,135){$q_3^2$}
\drawedge(ZF,ZG){$dec$}
\node(ZH)(110,135){$q_3^3$}
\drawedge(ZG,ZH){$dec$}
\node(ZI)(125,135){$q_3$}
\drawedge(ZH,ZI){$zero$}
%
\end{picture}
%
\caption{Weak determinization of one-counter machine}
\label{fig:weak-det}
%
\end{figure}
%
It can easily be proved by the way we build $M'$ and $T(\phi)$ from $M$ and $\phi$ that $M \models_F \phi$ (respectively $M \models_I \phi$) if and only if $M'\models_F T(\phi)$ (respectively $M' \models_I T(\phi)$) which allows us to deduce the following result.
%
\begin{proposition}\label{prop:wd}
The model-checking of one-counter machine with \freezeLTLdef (over finite and infinite runs) reduces to the model-checking of weakly deterministic one-counter machine with  \freezeLTLdef (over finite and infinite runs).
\end{proposition}

==> proof-lemma-bound-context.tex <==
(I) Ad absurdum, suppose that $j-i > K_1+K_1 K_2$. First, observe that $n_i < K_1$. 
Let $m$ be the minimal value in $\set{n_{K_1}, \ldots, n_{K_1+K_2-1}}$.
For all $l \geq K_1 + K_1 K_2$, we have $n_l \geq m + K_1 K_3 \geq K_1 K_3 > K_1$. Since 
$j \geq K_1 + K_1 K_2$, we deduce that $n_j > K_1$, 
which is in contradiction with  $n_i=n_j$.

(II) Ad absurdum, suppose that $(j-i) > K_2^2$. Remark that from a position $l \geq K_1$, we have for all $l' >l$, $n_{l'} \geq n_l -K_2/2$, in fact performing $K_2$ transitions after a position greater than $K_1$ amounts to add $K_3$ to every counter value. Consequently we can deduce that $n_j \geq n_{i+K_2^2} - K_2/2$. Since $n_{i+K_2^2}=n_{i}+K_2 K_3$, we conclude that 
$n_j \geq n_{i}+K_2 K_3 - K_2/2 \geq n_{i}+K_2- K_2/2 > n_i$, which leads to 
a contradiction. 

==> proof-lemma-move.tex <==
Let $\pair{i'}{pos_i}=[\pair{i}{\aregval}]$, $\pair{j'}{pos_j}=[\pair{j}{\aregval}]$ and $\pair{i''}{pos'}=\move([\pair{i}{\aregval}],(j-i))$.

First, we will show that $pos'=pos_j$. Suppose $K_3=0$, then we have that $pos'=pos_i$. 
Since for all $r \in \set{1, \ldots, N}$, $pos_i(r)=v(r)=pos_j(r)$, we deduce that $pos'=pos_j$. 
Now consider the case $K_3>0$. Then for $r \in  \set{1, \ldots , N}$, 
$pos'(r)=\set{\alpha-(j-i) : \alpha \in pos_i(r) , \alpha \geq (j-i)}$. 
Furthermore $pos_i(r)={\rm pos}_{\aautomaton}(i,\aregval(r))=\set{l \in \Nat : n_{i+l}=\aregval(r)}$. 
Let $l \in pos_i(r)$ such that $l \geq (j-i)$. 
Then $n_{j+l-(j-i)}=n_{i+l}=\aregval(r)$ and we can deduce that 
$l-(j-i) \in {\rm pos}_{\aautomaton}(j,\aregval(r))=pos_j(r)$. 
Now we suppose  that $l \in pos_j(r)$. Hence, $n_{j+l}=\aregval(r)$ and $n_{i+(i-j)+l}=v(r)$. 
If we denote $l+(j-i)$ by $l'$, then $l' \in pos_i(r)$ and since $l=l'-(j-i)$, we obtain that $l \in pos'(r)$.

We will now show that $i''=j'$. First, we suppose that $i+(j-i) \leq K_1+K_2-1$ then $i''=i+(j-i)=j$. Since $j \leq K_1+K_2-1$, we deduce $j'=j$. Second, we suppose that $i+(j-i) > K_1+K_2-1$. So we have that $i'' \equiv_{K_2} i + (j-i) \equiv_{K_2} j \equiv_{K_2} j'$ and since we have that $i'',j' \in \set{K_1, \ldots K_1 + K_2 - 1}$, we deduce that $i''=j'$.

==> proof-lemma-next.tex <==
Let $\pair{i'}{pos'}=[\pair{i}{\aregval}]$, $\pair{i''}{pos''}=[\pair{i+1}{\aregval}]$ and $\pair{j}{pos}=\movnext([\pair{i}{\aregval}])$.

First, we will show that $pos''=pos$. Suppose $K_3=0$, then we have that $pos=pos'$. 
Since for all $r \in \set{1, \ldots, N}$, $pos'(r)=v(r)=pos''(r)$, we deduce that $pos''=pos$. 
Now consider the case $K_3>0$. Then for $r \in  \set{1, \ldots , N}$, 
$pos(r)=\set{\alpha-1 : \alpha \in pos'(r) , \alpha >0}$. 
Furthermore $pos'(r)={\rm pos}_{\aautomaton}(i,\aregval(r))=\set{l \in \Nat : n_{i+l}=\aregval(r)}$. 
Let $l \in pos''(r)$ such that $l \geq 0$. 
Then $n_{i+1+l-1}=n_{i+l}=\aregval(r)$ and we can deduce that 
$l-1 \in {\rm pos}_{\aautomaton}(i+1,\aregval(r))=pos''(r)$. 
Now we suppose  that $l \in pos''(r)$. Hence, $n_{i+1+l}=\aregval(r)$. 
If we denote $l+1$ by $l'$, then $l' \in pos'(r)$ and since $l=l'-1$, we obtain that $l \in pos(r)$.

We will now show that $i''=j$. First, we suppose that $i+1 \leq K_1+K_2-1$ then $i''=i+1=j$. Second, we suppose that $i+1 > K_1+K_2-1$. So we have that $i'' \equiv_{K_2} i + 1 \equiv_{K_2} j $ and since we have that $i'',j \in \set{K_1, \ldots K_1 + K_2 - 1}$, we deduce that $i''=j$.



==> proof-lemma-polynomial.tex <==
 First, suppose that $K_3 = 0$. The run 
 $\arun_{\aautomaton}^{\omega}$ is of the form
 $$\pair{\aloc_0}{n_0} \cdots \pair{\aloc_{K_1-1}}{n_{K_1-1}}
 (\pair{\aloc_{K_1}}{n_{K_1}} \cdots \pair{\aloc_{K_1+
     K_2-1}}{n_{K_1+K_2-1}})^{\omega}.
$$
It is easy to see that for all $i \in \Nat$ and $m \not \in 
\set{n_0, \ldots, n_{K_1 + K_2 -1}}$, ${\rm pos}_{\aautomaton}(i,m) = \emptyset$. 
Moreover, 
\begin{itemize}
\itemsep 0 cm
\item for all $i,i' \geq K_1$ such that $i \equiv_{K_2} i'$ and register values
      $m \in \Nat$,
      we have ${\rm pos}_{\aautomaton}(i,m) =  {\rm pos}_{\aautomaton}(i',m)$,,
\item for every $i \leq K_1 + K_2 -1$,
      $$
\set{{\rm pos}_{\aautomaton}(i,m) \subseteq \Nat:  \ m \in \set{n_0, \ldots,n_i}}
      $$
      has cardinality at most $i + 1$.
\end{itemize}
%% Arn 310807
%%
%%Consequently, $\regvalues$ has cardinalities at most $(K_1 + K_2)^2 + K_2 + 1$. \\
Consequently, from the first point, we have
 $\regvalues=\set{{\rm pos}_{\aautomaton}(i,m): i \in \set{0, \ldots, K_1+K_2-1}, m \in \set{n_0, \ldots,n_i}} \cup \set{\emptyset}$  
whereas from  the second point, we get that its cardinality is at most $(K_1 + K_2)^2 + 1$.\\ 

Second, suppose that $K_3 > 0$ (and therefore $K_2 \leq \length{\locs}$). 
 The run 
 $\arun_{\aautomaton}^{\omega}$ is of the form below
$$\pair{\aloc_0}{n_0} \cdots \pair{\aloc_{K_1}}{n_{K_1}}
\cdots \pair{\aloc_{K_1+K_2}}{n_{K_1} + K_3} \cdots 
 \pair{\aloc_{K_1+2K_2}}{n_{K_1} + 2K_3} \cdots 
$$
The set $\set{n_j: j \geq 0}$ is therefore infinite
and $\aloc_{K1} = \aloc_{K_1 + K_2} = \aloc_{K_1 + 2K_2} = \ldots$. From lemma \ref{lemma-bound-context}, we deduce the following observations that will allow us to get the polynomial cardinality for $\regvalues$.
\begin{enumerate}
\itemsep 0 cm
\item The set $\set{{\rm pos}_{\aautomaton}(i,m): 0 \leq i \leq 
      K_1 + K_2^2, \ m \in \set{n_0, \ldots,n_i}}$ has at most $(1 + K_1 +  K_2^2)^2$ elements,
      which is polynomial in $\length{\locs}$.
\item For every $i \geq K_1 + K_2^2$, if $m \not \in \set{0, \ldots,K_1-1} \cup \set{n_{(i - K_2^2) + 1 }, \ldots, n_i}$,
      then ${\rm pos}_{\aautomaton}(i,m)$ is the empty set.
      %
      %Arn 040907
      %Indeed, performing $K_2$ transitions after a position greater than $K_1$ amounts to add $K_3 > 0$ to every counter value.
      %Hence, $\set{{\rm pos}_{\aautomaton}(i,m): \ m \in \set{n_0,
      %    \ldots,n_i}}$ has cardinality at most $K_2^2 + 1$.
      Hence, $\set{{\rm pos}_{\aautomaton}(i,m): \ m \in \set{n_0,
          \ldots,n_i}}$ has cardinality at most $K_2^2 + K_1 + 1$.
\item For all $i \geq K_1 + K_2^2$ and $m \in \set{n_{(i - K_2^2) + 1 }, \ldots, n_i}$,
      ${\rm pos}_{\aautomaton}(i+ K_2, m + K_3) = {\rm pos}_{\aautomaton}(i,m)$.
      Hence, for all $i,i' \geq K_1 + K_2^2$ such that $i \equiv_{K_2} i'$, 
      $$
      \set{{\rm pos}_{\aautomaton}(i,m): \ m \in \set{n_0, \ldots,n_i}} =
      \set{{\rm pos}_{\aautomaton}(i',m): \ m \in \set{n_0, \ldots,n_{i'}}}.
      $$
\end{enumerate}

==> proof-lemma-two-in-one.tex <==

(I) The proof is done by recurrence on $j$. First suppose that $j=1$. 
    The only point to check is that  $\aloc_{i+1}=\aloc_{i'+1}$, which is a simple consequence
of the determinism of $\aautomaton$. Indeed,  if there is only an incrementing transition from $\aloc_i$,
 then we get straightforwardly $q_{i+1}=q_{i'+1}$. Otherwise, if there are 
two transitions from $\aloc_i$, then  one is a decrementation and the other one is a zero-test.
The induction step is shown in a similar fashion. 

(II) Suppose $\pair{i}{\aregval} \equiv \pair{i'}{\aregval'}$.
The proof is by structural induction on $\aformulabis$.
%
\begin{itemize}
\itemsep 0 cm 
\item Case  $\aformulabis=q$: Since by definition $i \equiv i'$, we have that $q_i=q_{i'}$ and consequently $q_i=q$ iff $q_{i'}=q$.
%
\item Case  $\aformulabis=\uparrow_r $:
Since $n_i=v(r)$ iff $n_{i'}=v'(r)$, we have that $\arun_{\aautomaton}^{\omega}, i \models_{\aregval} \uparrow_r  $ iff
$\arun_{\aautomaton}^{\omega}, i' \models_{\aregval'} \uparrow_r $.
%
\item Case  $\aformulabis=\mynext \aformula$: Since $\pair{i}{\aregval} \equiv \pair{i'}{\aregval'}$, 
from Lemma~\ref{lemma-two-in-one}(I), 
we deduce that $\pair{i+1}{\aregval} \equiv \pair{i+1'}{\aregval'}$ and 
by (IH) we obtain  $\arun_{\aautomaton}^{\omega}, i+1 \models_{\aregval} \aformulabis$ iff
$\arun_{\aautomaton}^{\omega}, i'+1 \models_{\aregval'} \aformulabis$.
%
\item Case  $\aformulabis = \aformula_1 \until \aformula_2$: 
Suppose that there exists $j \geq 0$ such that $\arun_{\aautomaton}^{\omega}, i+j \models_{\aregval} \aformula_2$ and for all $0 \leq j' < j$, $\arun_{\aautomaton}^{\omega}, i+j' \models_{\aregval} \aformula_1$. 
Using Lemma~\ref{lemma-two-in-one}(I) and (IH),  
we deduce that $\arun_{\aautomaton}^{\omega}, i'+j \models_{\aregval} \aformula_2$ and for all $0 \leq j' < j$, $\arun_{\aautomaton}^{\omega}, i'+j' \models_{\aregval} \aformula_1$.
%
\item Case  $\aformulabis=\downarrow_r \aformula$:
We observe that if  $\pair{i}{\aregval} \equiv \pair{i'}{\aregval'}$ then $\pair{i}{\aregval[r \mapsto n_i]} \equiv 
\pair{i'}{\aregval'[r \mapsto n_i]}$. This is due to the fact that for 
$\alpha \geq 0,$ if $n_{i+a}=n_i$, then $n_i'=n_{i'+\alpha}$ (since $i \equiv i'$). 
By (IH), we get the desired result.
\end{itemize}

==> proof-lemma-until.tex <==
Let us be precise about $K_4$. 
Let $K_3 = 0$ [resp. $K_3 > 0$] and $\pair{i}{\asymbregval}$ be a symbolic
context.
\begin{description}
\itemsep 0 cm
\item[(I)] If $i < K_1$ then for every $\alpha \geq K_1 + 2 \times K_2$ [resp.  
            $\alpha \geq K_1 + (K_1 + 2) \times K_2$], there is $\beta < K_1 + 2 \times K_2$ 
            [resp. $\beta < K_1 + (K_1 + 2) \times K_2$] such that
           $$
           (1) \ \pair{\set{\move(\pair{i}{\asymbregval},j): 0 \leq j \leq \alpha-1}}{
                 \move(\pair{i}{\asymbregval},\alpha)} =
           $$
           $$
           \pair{\set{\move(\pair{i}{\asymbregval},j): 0 \leq j \leq \beta-1}}{
                 \move(\pair{i}{\asymbregval},\beta)}
           $$
\item[(II)]  If $i \geq K_1$ then for every $\alpha \geq 2 \times K_2$ [resp.  
            $\alpha \geq (K_2 + 2) \times K_2$], there is $\beta <  2 \times K_2$ 
            [resp. $\beta < (K_2 + 2) \times K_2$] such that $(1)$ holds true. 
\end{description}
 

We pose $K_4 = max(K_1 + (K_1 + 2) K_2, (K_2 + 2) K_2)$.

The above points are proved as follows by a simple case analysis.

First, we suppose that $K_3=0$. Let $i<K_1$ and $\alpha \geq K_1 + 2 \times K_2$. Then we define $\beta$ as the unique element of $\set{K_1+K_2, \ldots K_1+ 2 \times K_2 -1}$ such that $\alpha \equiv_{K_2} \beta$. If $i \geq K_1$ and $\alpha \geq 2 \times K_2$, we take $\beta$ as the unique element of $\set{K_2 , \ldots , 2 \times K_2 -1}$ such that $\alpha \equiv_{K_2} \beta$.

Second we suppose that $K_3 \geq 0$. Let $i<K_1$ and $\alpha < K_1 + (K_1 + 2) \times K_2$, then we define $\beta$ as the unique element of $\{K_1 + K_1 K_2 + K_2, \ldots , K_1 + K_1 K_2 + 2 \times K_2 -1\}$ such that $\alpha \equiv_{K_2} \beta$. If $i \geq K_1$ and $\alpha \geq (K_2 + 2) \times K_2$, then define $\beta$ as the unique element of $\{K_2 K_2 + K_2, \ldots ,  K_2 K_2 + 2 \times K_2 -1\}$ such that $\alpha \equiv_{K_2} \beta$.

It remains to check that $\beta$ satisfies the properties. 






==> proof-purif.tex <==
First, we give the formal description of how we build the one-counter automaton $\aautomaton_P$ from the one-counter automaton $\aautomaton=\triple{\locs,\aloc_I}{\delta}{F}$. We suppose $\locs=\set{\aloc_1,...,\aloc_n}$. Then  $\aautomaton_{P}=\triple{\locs',\aloc_I}{\delta}{F'}$ is defined as follows~:
%
\begin{itemize}
\item $\locs'=Q \cup \set{\aloc^0_i,\aloc^F_i}_{i \in \set{1,\ldots,n}} \cup \{\aloc_i^{j,k}\mid 1 \leq k \leq 2.j+2 \mbox{ and } 1 \leq j \leq i \mbox{ and } 1\leq i \leq n\}$
\item the relation $\delta'$ contains the following transitions~:
\begin{itemize}
\item For all $\aloc_i \in Q$, add $\aloc_i \step{\mathtt{inc}} \aloc^0_i$ and $\aloc^0_i \step{\mathtt{dec}} \aloc_i^{1,1}$ to $\delta'$;
\item For all $i \in \set{1,\ldots,n}$, for all $j \in \set{1,\ldots,i}$ and for all $k \in \set{1,\ldots,2.j-1}$~:
\begin{enumerate}
\item if $k<j+2$ add $\aloc_i^{j,k} \step{\mathtt{inc}} \aloc_i^{j,k+1}$ to $\delta'$;
\item if $k \geq j+2$ add $\aloc_i^{j,k} \step{\mathtt{dec}} \aloc_i^{j,k+1}$ to $\delta'$;
\end{enumerate}
\item For all $i \in \set{1,\ldots,n}$, for all $j \in \set{1,\ldots,i-1}$, add $\aloc_i^{j,2.j+2} \step{\mathtt{inc}} \aloc_i^{j+1,1}$

\item For all $i \in \set{1,\ldots,n}$, add $\aloc_i^{i,2.i+2}  \step{\mathtt{dec}} \aloc^F_i$ to $\delta'$;
\item For any transition $\aloc_i \step{a} \aloc_j \in \delta$, add a transition $\aloc^F_i \step{a} \aloc_j$ to $\delta'$.
\end{itemize}
\item And $F'=\set{q^F_i \mid q_i \in F}$.
\end{itemize}

==> under-construction.tex <==


We shall solve the model-checking checking by following an automata-based approach~\cite{Vardi&Wolper86}. 
Given an alternating word B\"uchi automaton $\aautomaton$, we write $\alang_{\omega}(\aautomaton)$
[resp. $\alang_{< \omega}(\aautomaton)$] to denote the set of infinite [resp. finite] words accepted
by $\aautomaton$. As usual, for runs accepting infinite runs, along each infinite branch there is an accepting
state occurring infinitely often. 


Let $\aformula$ be a formula in negative normal form built over disjunction $\vee$ and the release 
operator $\release$ (dual of $\until$). Observe that $\mynext$ and $\downarrow_{\aregister}$ are self-dual. 
Let $\aautomaton_{\aformula} = \triple{\aalphabet}{S, \astate_0, \rho}{F}$ be the following 
alternating B\"uchi automaton on infinite words for  $K_3 > 0$:

\begin{itemize}
\itemsep 0 cm 

\item $\aalphabet = \set{a}$ (1-letter alphabet).

\item $S$ is the set of locations of the form $\pair{\pair{i}{\asymbregval}}{\aformulabis}$
      where $\pair{i}{\asymbregval}$ is a symbolic context and $\aformula$ is a subformula of $\aformula$.

\item initial location $\astate_0 =  \pair{\pair{0}{\asymbregval_0}}{\aformula}$
      where $\asymbregval_0$ is thr symbolic register valuation representing the zero register valuation.

\item $F$ is the set of accepting states whose outermost connective of second component 
      is not until.

\item The transition relation $\rho$ is defined as follows:
      \begin{itemize}
      \itemsep 0 cm
      \item $\delta(\pair{\pair{i}{\asymbregval}}{\aloc}, a) = \top$ if $\aloc = \aloc_i$, otherwise   
            $\delta(\pair{\pair{i}{\asymbregval}}{\aloc}, a) = \perp$,
      \item  $\delta(\pair{\pair{i}{\asymbregval}}{\uparrow_{\aregister}}, a) = \top$ if $0 \in \asymbregval(\aregister)$,
             otherwise $\delta(\pair{\pair{i}{\asymbregval}}{\uparrow_{\aregister}}, a) = \perp$,   
      \item $\delta(\pair{\pair{i}{\asymbregval}}{\aformulabis \wedge \aformulabis'}, a) = 
             \delta(\pair{\pair{i}{\asymbregval}}{\aformulabis}, a) \wedge
             \delta(\pair{\pair{i}{\asymbregval}}{\aformulabis'}, a)$,
     \item $\delta(\pair{\pair{i}{\asymbregval}}{\aformulabis \vee \aformulabis'}, a) = 
             \delta(\pair{\pair{i}{\asymbregval}}{\aformulabis}, a) \vee
             \delta(\pair{\pair{i}{\asymbregval}}{\aformulabis'}, a)$,
      \item $\delta(\pair{\pair{i}{\asymbregval}}{\mynext \aformulabis}, a) = 
            \pair{\move(\pair{i}{\asymbregval},1)}{\aformulabis}$,
      \item $\delta(\pair{\pair{i}{\asymbregval}}{\downarrow_{\aregister} \aformulabis}, a) = 
             \delta(\pair{\pair{i}{\asymbregval [\aregister \leftarrow {\rm pos}_{\aautomaton}(i,n_i)] }}{\aformulabis}, a)$,
      \item  $\delta(\pair{\pair{i}{\asymbregval}}{\aformulabis \until \aformulabis'}, a) = 
             \delta(\pair{\pair{i}{\asymbregval}}{\aformulabis'}, a) \vee
             ( \delta(\pair{\pair{i}{\asymbregval}}{\aformulabis}, a) \wedge
               \pair{\move(\pair{i}{\asymbregval},1)}{\aformulabis \until \aformulabis'}$,
      \item  $\delta(\pair{\pair{i}{\asymbregval}}{\aformulabis \release \aformulabis'}, a) = 
             \delta(\pair{\pair{i}{\asymbregval}}{\aformulabis'}, a) \wedge
             ( \delta(\pair{\pair{i}{\asymbregval}}{\aformulabis}, a) \vee
               \pair{\move(\pair{i}{\asymbregval},1)}{\aformulabis \release \aformulabis'}$.
      \end{itemize}
\end{itemize}

When $K_3 = 0$, the clauses for $\downarrow_{\aregister}$ and $\uparrow_{\aregister}$ are the following:
\begin{itemize}
\itemsep 0 cm
\item  $\delta(\pair{\pair{i}{\asymbregval}}{\uparrow_{\aregister}}, a) = \top$ if $n_i = \asymbregval(\aregister)$,
             otherwise $\delta(\pair{\pair{i}{\asymbregval}}{\uparrow_{\aregister}}, a) = \perp$, 
 \item $\delta(\pair{\pair{i}{\asymbregval}}{\downarrow_{\aregister} \aformulabis}, a) = 
             \delta(\pair{\pair{i}{\asymbregval [\aregister \leftarrow n_i] }}{\aformulabis}, a)$.
\end{itemize}

Let $\aautomaton^{\pair{\pair{i}{\asymbregval}}{\aformulabis}}_{\aformula}$ be the alternating
B\"uchi automaton defined from $\aautomaton_{\aformula}$ with initial location 
$\pair{\pair{i}{\asymbregval}}{\aformulabis}$. 

\begin{lemma} Let $i \in \Nat$ and $\aregval$ be a register valuation with range $\set{n_0, \ldots, n_i}$.
For every subformula $\aformulabis$ of $\aformula$, $\arun_{\aautomaton}^{\omega}, i \models_{\aregval} \aformulabis$
iff  $\aautomaton^{\pair{\pair{i}{\asymbregval}}{\aformulabis}}_{\aformula}$ accepts an infinite run.
\end{lemma}

The proof is by structural induction. 

The nonemptiness problem for hesitant alternating word automata
over a 1-letter alphabet can be solved in space $\mathcal{O}(m \ log^2 \length{S})$
\cite{Bernholtz&Vardi&Wolper94}
where $m$ is the number of sets in the partition $S_1,\ldots, S_m$ equipped
with a partial order $\leq$ such
that 
\begin{itemize}
\itemsep 0 cm
\item $S_1 \uplus S_2 \uplus \cdots \uplus S_m = S$ and if $\astate' \in \rho(\astate, a)$ with $\astate \in S_i$ and
      $\astate' \in S_j$, then $S_j \leq S_i$,
\item for each $j$, (either $S_j \subseteq F$ or $S_j \cap F \neq \emptyset$) and $S_j$ is transient.
\end{itemize}
This will allow us to characterize precisely the complexity of model-checking.




